CrossRectify: Leveraging Disagreement for Semi-supervised Object Detection

Semi-supervised object detection has recently achieved substantial progress. As a mainstream solution, the self-labeling-based methods train the detector on both labeled data and unlabeled data with pseudo labels predicted by the detector itself, but their performances are always limited. Through experimental analysis, we reveal the underlying reason is that the detector is misguided by the incorrect pseudo labels predicted by itself (dubbed self-errors). These self-errors can hurt performance even worse than random-errors, and can be neither discerned nor rectified during the self-labeling process. In this paper, we propose an effective detection framework named CrossRectify, to obtain accurate pseudo labels by simultaneously training two detectors with different initial parameters. Specifically, the proposed approach leverages the disagreements between detectors to discern the self-errors and refines the pseudo label quality by the proposed cross-rectifying mechanism. Extensive experiments show that CrossRectify achieves outperforming performances over various detector structures on 2D and 3D detection benchmarks.

==> 0_abstract-bak.tex <==
\begin{abstract}
Semi-supervised object detection has recently achieved substantial progress. 
%
As a mainstream, the self-labeling-based method trains the detector on both labeled
data and unlabeled data with pseudo labels predicted by the detector itself.
%
However, the performances are always limited.
%
In this paper, we point out two limitations in self-labeling, that are the misclassified pseudo labels can be neither realized nor rectified by the detector itself.
%
Such limitations lead the detector to over-fit on self-errors, and the detection performance can be hurt even worse by self-errors than by random-errors. 
%
Thus we propose an effective training framework named CrossRectify, where two detectors are simultaneously trained and the disagreements are leveraged to realize and rectify the potential errors predicted by each single detector.
%
Moreover, we conduct quantitative experiments to show our superiority on improving pseudo label quality.
%
Our method achieves outperforming performances over various detector structures
on both 2D and 3D object detection datasets.
\end{abstract}

==> 0_abstract-more-than-150.tex <==
\begin{abstract}
Semi-supervised object detection (SSOD) has achieved substantial progress in recent years, which leverages a few labeled data and a large amount of unlabeled data to train detector models.
%
As a mainstream solution, the self-labeling-based SSOD methods train the detector on both labeled data and unlabeled data with pseudo labels predicted by the detector itself.
%
However, the performances are always observed limited.
%
In this paper, we first point out two limitations in self-labeling, that are the misclassified pseudo labels can be neither realized nor rectified by the detector itself.
%
Such limitations lead the detector to over-fit on self-errors, % and hinder the detection performance.
%
and we prove by experiments that the detection performance can be hurt even worse by self-errors than by random-errors.
%
To overcome these issues, we propose an effective and general training framework named CrossRectify, where two detectors with same structure but different initialization are trained simultaneously. 
%
Specifically, the inter-disagreements on the same objects between two detectors are utilized to recognize the potential errors predicted by each single detector, and to further rectify errors by making comparison on probability scores.
%
Moreover, we conduct quantitative experiments to show the superiority of CrossRectify on improving pseudo label quality when compared with other similar works.  % theoretical analysis and 
%
Our method achieves the state-of-the-art performances over various detector structures on both 2D and 3D semi-supervised object detection benchmark datasets, including Pascal VOC, MS-COCO, and SUN-RGBD.
%
The code for reproducing main results is available at \url{https://github.com/machengcheng2016/CrossRectify-SSOD}.
\end{abstract}

==> 1_introduction-bak.tex <==
\section{Introduction}
\label{sec:intro}
% Here are two sample references: \cite{Feynman1963118,Dirac1953888}.
The success of deep learning has greatly promoted the development of object detection approaches~\cite{SSD,FasterRCNN,bosquet2021stdnet,wang2021multi,kong2021spatial,zhang2021cadn}, and a large amount of labeled data is essential to the training process of object detectors.
%
However, as illustrated in \cite{kuznetsova2020open}, it is always labor-intensive and expensive to acquire a large amount of labeled data with bounding-box-level annotations. 
%
In comparison, unlabeled data are much easier and cheaper to collect.
%
Therefore, semi-supervised object detection~\cite{SSOD} is recently investigated to reduce the cost of data annotating, which leverages only a few labeled data and a large amount of unlabeled data to train object detectors.





Semi-supervised object detection (SSOD) has achieved significant progress in recent years, and one of the mainstream SSOD solutions is based on the self-labeling scheme~\cite{self-labeling}.
%
The core idea of self-labeling scheme is to first utilize the current detector to predict pseudo bounding boxes for unlabeled data in each training iteration, then conducts detector training with both labeled data and pseudo-labeled data. 
%
However, compared with fully-supervised baselines, the performance increments brought by the self-labeling-based methods are always observed limited, which are only 0.40\% and 0.46\% absolute AP$_{50}$ gains without and with data augmentation (as shown in Fig.~\ref{fig:first-page}).
%
Since the key to the success of SSOD is the pseudo label quality, all existing self-labeling-based SSOD methods select the predicted bounding boxes with high confidence scores as pseudo labels. 
%
The rationale behind such process is that higher-confidence boxes are more likely to be correctly classified than lower-confidence ones. 
%
However, through experimental analysis, we point out two inherent limitations of the self-labeling training scheme, that are 
(a) \textit{some of high-confidence boxes may still be misclassified and cannot be discerned by the detector itself}, 
(b) \textit{those incorrect pseudo boxes cannot be rectified by the detector itself}.
These two limitations will lead the detector to over-fit on self-errors, and we prove by experiments that the detection performance will be hurt even worse by self-errors than by random-errors.  
%
Such over-fitting issue suppresses the potential of self-labeling scheme and finally results in insignificant performance increments.
%
% More experimental analysis on self-labeling-based SSOD methods are presented in Section~\ref{sec:over-fitting in sela}.


\input{Figures/first-page}

Since one single detector can neither discern nor rectify the misclassified pseudo bounding boxes, it is reasonable to introduce the guidance from other separate detectors to the training process.
%
Recently, a few works \cite{CoTraining,ke2019dual,wei2020combating,coteaching+} illustrate the fact that two differently initialized models with an identical structure can still yield diverse results on the same input data during the training process. 
%
Inspired by this fact, in this paper, we propose an effective and general training framework for semi-supervised object detection named CrossRectifiy to address the problems mentioned above. 
%
In CrossRectify, two detector models with same structure but different initialization are trained simultaneously, and each model takes the high-confidence predictions from both models for pseudo label generation. 
%
Intuitively, the disagreements on the same object between two detectors can reveal the potential misclassification. 
%
Besides, we leverage the inter-model disagreements to rectify the possible errors by comparing probability scores and further alleviate the over-fitting issue in self-labeling scheme. 
%
The proposed CrossRectify algorithm is detailed in Section \ref{sec:CrossRectify}.




%
Note that a few recent works also attempt to overcome the over-fitting problem in self-labeling-based SSOD methods. 
%
For instance,~\cite{STAC,DataUncertainty,UnbiasedTeacher,HumbleTeacher,SoftTeacher} follow the teacher-student mutual learning framework~\cite{MeanTeacher} and utilize the separate teacher model to generate pseudo labels in an offline or online way.
%
Besides,~\cite{InstantTeaching} adopts the idea of co-training framework~\cite{wei2020combating,CoTraining,ke2019dual} to train two detector models simultaneously, and utilizes two sets of predicted bounding boxes to improve the pseudo label quality. 
% 
To compare with these similar works, we conduct quantitative experiments and show the superiority of our CrossRectify on improving the pseudo label quality (see Section \ref{sec: discussions}).


%
We carry out extensive experiments on both 2D and 3D semi-supervised object detection tasks to verify the effectiveness and versatility of the proposed CrossRectify method. As illustrated in Section \ref{sec: results}, our method obtains consistent and substantial improvements compared with the state-of-the-art SSOD methods on the Pascal VOC, MS-COCO, and SUN-RGBD benchmark datasets.




Our main contributions are summarized as follows:
\begin{enumerate}[1)]
\item We point out that two inherent limitations in self-labeling-based SSOD methods will lead the detector to over-fit on self-errors, and self-errors will hurt the detector performance even worse than random-errors. 
\item We propose the CrossRectify algorithm to address the over-fitting problem, using the inter-model disagreements. We also conduct quantitative experiments to show the superiority of our CrossRectify on improving pseudo label quality, compared with other similar works.
\item Extensive experiments carried on both 2D and 3D SSOD tasks verify the effectiveness and versatility of the proposed CrossRectify method.
\end{enumerate}

==> 3_problem_analysis_bak.tex <==
\section{Problem Analysis}
\label{sec:methodology}

In this section, we first introduce the preliminaries in semi-supervised object detection (SSOD), then analyze the inherent limitations of self-labeling-based SSOD methods.



\subsection{Preliminaries}
\label{sec:preliminaries}
Under the semi-supervised setting, an object detector $f$ is trained on a labeled dataset $D_l= \{\boldsymbol x_i^l, \boldsymbol y_i^l\}_{i=1}^{N_l}$ with $N_l$ samples and an unlabeled dataset $D_u= \{\boldsymbol x_j^u\}_{j=1}^{N_u}$ with $N_u$ samples.
%
For a labeled image $\boldsymbol x^l$, its annotation $\boldsymbol y^l=(\boldsymbol c, \boldsymbol t)$ contains the category labels $\boldsymbol c$ and coordinates $\boldsymbol t$ of all foreground objects.
%



Overall, the detector model $f$ is optimized by minimizing the supervised loss $L_S$ on labeled data and unsupervised loss $L_U$ on unlabeled data, formulated as:
% \vspace{-1mm}
\begin{flalign}
L = L_{S} + \lambda_{U} \cdot L_{U},
\label{eq: loss_total}
% \vspace{-1mm}
\end{flalign}
where $\lambda_{U}$ denotes the weight factor.
%
Generally, the supervised loss $L_S$ consists of the classification loss $l_{cls}$ and coordinate regression loss $l_{reg}$:
% \vspace{-1mm}
\begin{flalign}
L_S = l_{cls}\big(f_{cls}(\boldsymbol x^l), \boldsymbol c \big)+l_{reg}\big(f_{loc}(\boldsymbol x^l), \boldsymbol t \big),
\label{eq: supervised loss}
% \vspace{-1mm}
\end{flalign}
where $f_{cls}(\boldsymbol x^l)$ and $f_{loc}(\boldsymbol x^l)$ stand for probabilities and coordinates predicted by the classification and localization branch of detector $f$, respectively.




In each training iteration, the self-labeling-based SSOD method utilizes the current detector to predict bounding boxes on the unlabeled inputs $\boldsymbol x^u$, and then selects the pseudo labels $\hat{\boldsymbol y}$ with confidence larger than the threshold $\tau$, and finally computes the unsupervised loss:
% \vspace{-1.0mm}
\begin{flalign}
L_U = l_{cls}\big(f_{cls}(\boldsymbol x^u), \hat{\boldsymbol c}\big)
    + l_{reg}\big(f_{loc}(\boldsymbol x^u), \hat{\boldsymbol t}\big),
\label{eq: self-labeling}
% \vspace{-1mm}
\end{flalign}
where $\hat{\boldsymbol y}=(\hat{\boldsymbol c}, \hat{\boldsymbol t})=\big(\argmax f_{cls}(\boldsymbol x^u), f_{loc}(\boldsymbol x^u)\big)$
and $\max f_{cls}(\boldsymbol x^u) > \tau$ are correspondingly satisfied.

%where $w(\boldsymbol x^u)$ denotes the confidence thresholding mask, with $w(\boldsymbol x^u)$ being 1 if $\max f_{cls}(\boldsymbol \alpha(\boldsymbol x^u)) > \tau$ else 0.

As the special case of self-labeling training, the consistency-regularization-based methods introduce weak data augmentation $\alpha(\cdot)$ and strong data augmentations $A(\cdot)$, and the Eq.~(\ref{eq: self-labeling}) is updated as:
% \vspace{-1mm}
\begin{flalign}
L_U = l_{cls}\big(f_{cls}(A(\boldsymbol x^u)),\argmax f_{cls}(\alpha(\boldsymbol x^u)) \big) 
    + l_{reg}\big(f_{loc}(A(\boldsymbol x^u)), f_{loc}(\alpha(\boldsymbol x^u)) \big).
\label{eq: consistency regularization}
% \vspace{-1mm}
\end{flalign}
Note that as for the consistency regularization, the loss term Eq.~(\ref{eq: consistency regularization}) can be computed on both labeled and unlabeled data, and the strong augmentations can also boost the performances of fully-supervised training~\cite{ISD}.
Accordingly, the total loss in Eq.~(\ref{eq: loss_total}) is augmented as $L = L_{S} + \lambda_{U} \cdot \big(L_U(\boldsymbol x^l) + L_U(\boldsymbol x^u)\big)$, and the fully-supervised baseline is trained by optimizing $L = L_{S} + \lambda_{U} \cdot L_U(\boldsymbol x^l)$.


\input{Tables/self-labeling-based-performances}

\subsection{Limitations of Self-labeling}
\label{sec:over-fitting in sela}
To verify the performances of existing self-labeling-based SSOD methods, we conduct experiments on the Pascal VOC benchmark dataset~\cite{VOC} based on the SSD300 structure~\cite{SSD}. 
%
We use the trainval set of VOC07 as labeled data and trainval set of VOC12 as unlabeled data, and finally report the AP$_{50}$ performance on the test set of VOC07. 
%
The confidence threshold $\tau$ is fixed as 0.5, similar with \cite{CSD} and \cite{ISD}.
%
For comparison, we conduct fully-supervised training with same hyper-parameters (batch size, iteration number, \etc) as baseline. 
%
As shown in Table~\ref{tab: self-labeling-based-performances}, the AP$_{50}$ increment brought by self-labeling methods is only 0.40\%.
%
Besides, we test with two representative consistency-regularization-based methods, namely CSD~\cite{CSD} and ISD~\cite{ISD}. 
%Here we conduct the fully-supervised training by optimizing $L = L_{S} + \lambda_{U} \cdot L_U(\boldsymbol x^l)$, in order to observe the absolute performance increment brought by unlabeled data. 
%
Again, the detection results achieve only 0.46\% absolute AP$_{50}$ gains over the baseline, which illustrates the inefficiency of self-labeling training scheme.


\input{Tables/overfitting-performances}
\input{Figures/confidence-thresholding}


To know the reason behind such phenomenon and find out possible solutions, we look up to the ground-truth category labels of all pseudo bounding boxes for in-depth analysis.
%
Although all existing self-labeling-based SSOD methods conduct confidence thresholding to ensure the pseudo label quality, Fig.~\ref{fig:confidence-threshold}(a) illustrates that part of high-confidence pseudo bounding boxes can also be misclassified. 
%
We name these incorrect boxes ``self-errors'' for clarity.
%
Since all pseudo boxes are predicted by the detector, it is impossible for the detector itself to discern the self-errors, which turns out to be the inherent limitation of the self-labeling process. 
%
We further conduct an experiment to illustrate how much can such limitation affect the detection performance:
%
in each training iteration, if we use the correct pseudo bounding boxes and discard the incorrect ones for training, the AP$_{50}$ result will increase from 72.13\% to 74.03\% (see the 2nd and 5th rows in Table~\ref{tab: overfitting-analysis}).
%
Besides, we note that the detection performance cannot be improved by naively increasing the confidence threshold $\tau$.
%
As shown in Fig.~\ref{fig:confidence-threshold}(a) and (b), the precision of pseudo bounding boxes increases from 71\% to 91\% as the threshold increases from 0.4 to 0.8,
%
while a large threshold can also overkill the correct pseudo boxes and waste the unlabeled training data. 
%
Correspondingly, we conduct self-labeling training under three settings of the threshold $\tau$: (i) fixed as 0.5, (ii) fixed as 0.8, (iii) rising from 0.5 to 0.8 gradually during the whole training process. 
%
As displayed in Table~\ref{tab: overfitting-analysis} (from 2nd row to 4th row), the trade-off between precision and recall leads to similar final performances (about 72.1\% AP$_{50}$).
%We 
%
%Such phenomenon illustrates the importance of discerning self-errors.


Since the self-errors cannot be discerned during the self-labeling process, it is also impossible for the detector to rectify them, which turns out to be the second limitation of the self-labeling process. 
%
In each training iteration, if we utilize the ground-truth (GT) category labels for all pseudo bounding boxes, the AP$_{50}$ result will increase to 74.86\%, obtaining a 3.13\% absolute gain rather than 0.40\% (see the penultimate row in Table~\ref{tab: overfitting-analysis}). 
%
Such phenomenon shows the effectiveness of pseudo label rectification.
%
Besides, we find another interesting phenomenon: 
%
if we replace the category labels of self-errors with random category labels (dubbed random-errors) for self-labeling training, the final performance will increase to 73.87\% (see the third row from the bottom in Table~\ref{tab: overfitting-analysis}). 
%
We also conduct experiments over the Faster-RCNN-FPN structure~\cite{FasterRCNN} and observe the similar trend: the AP$_{50}$ result of self-labeling will be increased with 0.2\%, by the process of replacing the labels of self-errors with random labels during training.
%
Such phenomena imply that detector model can be misguided more severely by self-errors than random-errors. 
%The key to the success

Based on the above experimental analysis, we draw that two inherent limitations in self-labeling-based SSOD methods will lead the detector to be misguided by self-errors, and self-errors will hurt the detector performance even worse than random-errors.







\begin{comment}
\vspace{-1.0mm}
\begin{flalign}
\hat{\boldsymbol y}=(\hat{\boldsymbol c}, \hat{\boldsymbol t})=\big(\arg\max f_{cls}(\boldsymbol x^u), f_{loc}(\boldsymbol x^u)\big)
\label{eq: y=(c,t)}
\end{flalign}

\arg\max f_{cls}(\boldsymbol x^u)

\vspace{-1.0mm}
\begin{flalign}
L_U &= l_{cls}\big(f_{cls}(A(\boldsymbol x^u)),\arg\max f_{cls}(\alpha(\boldsymbol x^u)) \big) \nonumber\\  
    &+ l_{reg}\big(f_{loc}(A(\boldsymbol x^u)), f_{loc}(\alpha(\boldsymbol x^u)) \big),
\label{eq: self-labeling}
\end{flalign}
, and 
\end{comment}

==> Figures/visualization-one.tex <==
\begin{figure}[t]
\centering
{
\includegraphics[width=0.95\linewidth]{Images/visualizations/visualizations_one-crop.pdf}
}
%\vspace{-2mm}
\caption{The visual comparisons between Self-Labeling (the first row) and the proposed CrossRectify method (the second row) on MS-COCO under 1\% degree of supervision.
  (For color discrimination in this figure, please refer to the online version of this article.)}
\label{fig: visualization}
%\vspace{-2mm}
\end{figure}

==> Tables/extension-to-four-models.tex <==
\begin{table}[t]
\centering
%\scriptsize
%\vspace{1mm}
\scalebox{0.95}{
\begin{tabular}{ c c c c c c}
\hline
Model & Dataset & Index & Single & Average & Merged
\\ \hline
\multirow{6}{*}{SSD300}  &\multirow{6}{*}{VOC} & detector \#1     &   73.67   &   \multirow{2}{*}{73.65}  &   \multirow{2}{*}{74.83}
\\ 
&&detector \#2     &   73.63   &                           &
\\ \cline{3-6}
&&detector \#1     &   73.60   &   \multirow{4}{*}{73.71}  &   \multirow{4}{*}{75.84}
\\ 
&&detector \#2     &   73.71   &                           &
\\ 
&&detector \#3     &   73.80   &                           &
\\ 
&&detector \#4     &   73.73   &                           &
\\\hline
\end{tabular}
}
\vspace{-1mm}
\caption{Extension from two-detector to four-detector cross teaching. Single denotes the mAP result of each detector. Average denotes the average mAP of all detectors. Merged denotes the mAP of merged predictions by applying the weighted box fusion from all detectors.}
\label{tab: extension-to-four-models}
\vspace{-2mm}
\end{table}
